Toward Fairness Through Fair Multi-Exit Framework for Dermatological Disease Diagnosis

Fairness has become increasingly pivotal in medical image recognition. However, without mitigating bias, deploying unfair medical AI systems could harm the interests of underprivileged populations. In this paper, we observe that while features extracted from the deeper layers of neural networks generally offer higher accuracy, fairness conditions deteriorate as we extract features from deeper layers. This phenomenon motivates us to extend the concept of multi-exit frameworks. Unlike existing works mainly focusing on accuracy, our multi-exit framework is fairness-oriented; the internal classifiers are trained to be more accurate and fairer, with high extensibility to apply to most existing fairness-aware frameworks. During inference, any instance with high confidence from an internal classifier is allowed to exit early. Experimental results show that the proposed framework can improve the fairness condition over the state-of-the-art in two dermatological disease datasets.

==> Section/Experimental_Settings.tex <==
\subsection{Datasets}

In this work, we evaluated our method on two disease classification datasets ISIC 2019 challenge \cite{Combalia2019BCN20000DL} \cite{Tschandl2018TheHD} and the Fitzpatrick-17k dataset \cite{Groh2021EvaluatingDN} . ISIC 2019 challenge contains 25,331 images in 9 diagnostic categories of target labels. We took the gender labels as our sensitive attribute.
The Fitzpatrick-17k dataset contains 16,577 images in 114 skin conditions of target labels and defines the skin tone labels as the sensitive attributes. The skin tones are categorized into six levels from 1 to 6. The smaller the value, the lighter the skin. Therefore, we categorize levels 1 to 3 as light skin and 4 to 6 as dark skin. 

\subsection{Evaluation Metrics}
\label{sec:evaluation_metrics}
Several fairness metrics are proposed to evaluate the degree of fairness in classification task. Demographic parity \cite{dwork2012fairness} and equalized odds (EO) \cite{hardt2016equality,dwork2012fairness} are two well-known fairness criterion. We first define an input feature $X \in \mathbb{R}^d$ with sensitive attribute $A$, ground truth target class $Y$, and the predicted target class $\hat{Y}$. Demographic parity is satisfied if 
\begin{equation}
\label{eq.DEO}
P(\hat{Y} = 1|A = 0) = P(\hat{Y} = 1|A = 1).
\end{equation}
The drawback of demographic parity is that the classifier could achieve the fairness condition by adjusting the proportion of correct rate of two sensitive attributes through misclassifying some instances. On the other hand, EO forces the true positive rate and the false positive rate along different groups to be equal, that is, 
\begin{equation}
\label{eq.EO}
P(\hat{Y} = 1|A = a, Y = y) = P(\hat{Y} = 1|A = b, Y = y)
\end{equation}
We evaluate our model by multi-class equalized opportunity (Eopp) and equalized odds (Eodd) to quantify the fairness performance \cite{Hardt2016EqualityOO}. The equalized opportunity has two metrics to evaluate the correct prediction. Eopp0 indicates the difference between the two groups' true negative rate (TNR), and Eopp1 illustrates the difference between the two groups' true positive rate (TPR). Equalized odds is the summation of two groups' true positive rate difference and false positive rate difference, which can also address unfair wrong prediction of the model.
% where $y \in \{0, 1\}$, and $a, b \in A$. This metric addresses unfair wrong prediction of the model, and therefore EO will be the suitable fairness metric to evaluate our model. We calculate the degree of EO by calculating the disparity of the $TPR$ and $FPR$ alone different sensitive attributes as follows:
% \begin{equation}
% \label{eq.EO_equation}
%     \sum_{k=1}^{K} |TPR_{k}^{1} - TPR_{k}^{0} + FPR_{k}^{1} - FPR_{k}^{0}|
% \end{equation}
% where $TPR_{k}^{a}$ and $FPR_{k}^{a}$ are the True Positive Rate and the False Positive Rate respectively of target class $k$ and sensitive attribute $a$, this equation can also extend to multi-attribute cases. In conclusion, the optimal EO score becomes $0$ when the True Positive Rate and the False Positive of each target and sensitive class are the same. It indicates that a lower EO represents the prediction is fairer.

% Following most related works, we report EO and accuracy (Acc.) of all experiments in section \ref{sec:result}. 


\subsection{Implementation Details}
We utilize Resnet-18 as the backbone of every state-of-the-art and the baseline CNN used in our experiments. 
In the training phase, the data is augmented by random flipping, rotation, and scaling before being fed into the model. The network is trained for 200 epochs using SGD optimizer \cite{ruder2016overview} with an initial learning rate set as 0.01. We attach three internal classifiers at the end of each residual block. The internal classifier contains one adaptive average pooling layer and a two layer MLP. As introduced in Section \ref{sec:method_main}, the modified loss function in the multi-exit training framework is a weighted summation of the loss from each internal classifier. The coefficients, $\alpha_1$, $\alpha_2$, $\alpha_3$, and $\alpha_f$, are set to $0.3$, $0.45$, $0.6$, and $0.9$, respectively. We set the confidence threshold $\theta=0.85$ for the early exit policy at the inference phase.  

To show that our scheme can be widely applied to most existing frameworks, we conduct experiments on four baselines selected from state-of-art approaches for fairness-aware learning: LNL \cite{kim2019learning}, HSIC \cite{quadrianto2019discovering}, MFD \cite{jung2021fair}, and FSCL \cite{park2022fair}. All the baselines are reproduced by following the recommended hyperparameter settings of the original papers or resources.
 
\input{Table/Compare_SOTA_CelebA}
% \label{sec:implementation_details}
% \subsubsectionion{ME-CNN}

% \subsubsectionion{\emph{ME-LNL}} 
% We substitute the network {g \circ h} in to ME-CNN with three internal classifiers  and implemented the \emphh{h} with single fully connected layer. For the hyperparameter  





==> Section/Motivation_.tex <==
\begin{figure}[h]
% \setlength{\belowcaptionskip}{-20pt} 
\begin{center}

\includegraphics[width=0.99\linewidth]{Fig/Motivation.png}

\caption{Equalized odds (EO) and accuracy (Acc.) for the internal layers of the conventional ResNet on CelebA (a-b) and UTK Face (c-d) dataset. Note that lower EO represents fairer. (a) and (c) are the results using ResNet-18, while (b) and (d) use the ResNet-50. T and S stand for target and sensitive attributes, respectively. In the CelebA dataset, $a$, $e$, $m$, and $y$ represent \emph{attractiveness}, \emph{bags-under-eyes}, \emph{male}, and \emph{young}, respectively. For the UTK Face dataset, $A$ and $E$ are the \emph{Age} and \emph{Ethnicity}, respectively.
}
\label{Fig.Motivation}
\end{center}
\end{figure}

As shown in Fig. \ref{Fig.Motivation}, we observe that despite the features from a deep layer of a neural network bring high accuracy in classification, they cause fairness condition to deteriorate. We report the equalized odds (EO) and accuracy (Acc.) of ResNet-18 and ResNet-50 on the CelebA and the UTK Face dataset. We first trained a vanilla CNN, and froze the backbone. Then, we trained 3 MLP classifiers with the features from each residual module (i.e., Conv2\_x, Conv3\_x, Conv4\_x, Conv5\_x).

For CelebA dataset, in the experiments of the ResNet-18 (Fig. \ref{Fig.Motivation}(a)) and the ResNet-50 (Fig. \ref{Fig.Motivation}(b)), both the equalized odds (EO) and accuracy (Acc.) increase when the features are extracted from deeper layers. When comparing the accuracy between conv2\_x and the final layer in ResNet-18, the final layer has improved 6\% on average. However, the EO also increases over six times larger on average. As for the ResNet-50, the accuracy increased by about 16\%, and the EO increased more than eight times larger on average.

In Fig. \ref{Fig.Motivation}(c) and (d), results on UTK Face dataset again show a similar trend on the increasing EO and accuracy from shallow to deep layers. The ResNet-18 (Fig. \ref{Fig.Motivation}(c)) shows a 47\% improvement in accuracy with 1.7 times higher EO from the shallow layer (conv2\_x) to the deeper layer (Final layer). As for the ResNet-50 (Fig. \ref{Fig.Motivation}(d)), accuracy increases about 52\% and EO increases over 2.3 times.

As higher EO stands for larger bias (unfair) of the predicted result, intuitively, choosing the result at a shallow layer for final prediction could ameliorate the bias condition of the model. Our extensive experiments demonstrate that our observation could be applied to different network architectures and datasets.


==> Section/Related_Works.tex <==
\subsection{Early Exit Networks} % 改叫early exit networks?.
The early exit network is designed to reduce the computational resource during the model inference time while enhancing the model accuracy. With the early exit scheme, early exit branches will be attached to DNN. When the inference phase, the instances will stop inferencing and leave the model from different branches following the pre-defined early exit rules or criteria. BranchyNet \cite{Teerapittayanon2016BranchyNetFI}  calculates entropy at each branch after obtaining the result and exits if the entropy of the predicted result is less than the threshold value. Shallow-Deep Networks \cite{Kaya2019ShallowDeepNU} calculates the softmax score of each internal classifier's prediction and takes the maximum probability value as the confidence score. Once the score exceeds the threshold during the forward passing, the instance will exit from the branch prematurely, and the model further mitigates the "overthinking" problem of DNNs. \cite{schwartz-etal-2020-right} leveraged the early exit inference scheme of \cite{Kaya2019ShallowDeepNU} and applied a confidence-based strategy to the NLP task. \cite{Zhou2020BERTLP} makes predictions using adjacent layers and stops inference when the predicted value of the internal classifier remains constant in a given inference unit times. We borrow the architecture of \cite{Kaya2019ShallowDeepNU} and the confidence-based early exit strategy to achieve fairness classification. To our best knowledge, we are the first work that leverages the early exit technique to improve fairness.


\subsection{Bias Mitigation Methods}
Bias mitigation methods are designed to reduce the native bias in the dataset to reduce the chance of unfair prediction. There are largely three avenues for current debiased strategy, including pre-processing, in-processing, and post-processing. 
(1) Pre-processing strategies usually remove the information which may cause "discrimination" from training data before training. \cite{Kamiran2011DataPT} use different weight to neutralize the effect of the sensitive information in training phase and present the experiments result on real-life data. \cite{Ngxande2020BiasRI} and \cite{Lu2020GenderBI} achieve fairness via data pre-process methods including data generation and data augmentation.

In-processing method usually modify on-the-shelf model architecture, loss function, and model regularization to achieve fairness goal. \cite{Wang2020TowardsFI} used domain-independent training technique to improve fairness. Adversarial training mitigates the bias through adversarially trains an encoder and classifier to learn a fair representation. \cite{Zhang2018MitigatingUB} adversarially cooperate a predictor and a adversary to make accurate prediction while removing the sensitive attributes from the representation. \cite{kim2019learning} unlearned the bias of the dataset with the proposed regularization and trained the model in a adversarial fashion.
Disentangled representation forces the encoder abandon the information of sensitive attributes and thus achieve fairness.  

Post-processing method aims to calibrate the model's output to enhance fairness. They need to use sensitive attribute and prediction distribution to modify the previous distribution result. The \cite{Hardt2016EqualityOO} reveals the limit of demographic parity and give a new metric to fairness, equalized odds, and show how to adjust the learned prediction. \cite{Zhao2017MenAL} used Lagrangian relaxation to designed an inference algorithm which decrease bias but maintain performance in the meantime.


%% ?????
% However, those pre-processing and post-processing methods are not suitable for medical image diagnosis task because they need to remove or access sensitive attribute during experiment, it may influence the diagnosis, so our method focus on improving fairness in training phase. Moreover, out method can achieve fairness without knowing sensitive attribute in the training time, which is a "fairness through unawareness" technique.

However, most pre-processing and post-processing methods are unsuitable for medical image diagnosis tasks because they are required to remove or access sensitive attributes during the experiment, which are not practical. As a result, our method focus on improving fairness in the training phase. Moreover, our method can achieve fairness without knowing sensitive attributes during training, which is a "fairness through unawareness" technique.

==> Section/Related_work.tex <==
\subsection{Multi-exit Networks and Early Exit Policy} % 改叫early exit networks?.
The multi-exit network improves accuracy at the shallow layer by adding loss constraints to internal exit branches. Early exit branches reduce computational resources while enhancing accuracy \cite{kaya2019shallow}. In the inference phase, instances stop inference and leave the model from different branches based on pre-defined rules. Different models use various exit strategies, such as entropy-based or confidence-based scoring, to exit the model\cite{teerapittayanon2016branchynet,kaya2019shallow}. Recently, power\cite{shrestha2022occamnets} shows that multi-exit structure can mitigate dataset bias and improve model predicted. In this paper, we uses the confidence-based early exit strategy to ensure that the early exit instance is confident enough to be correct. To our best knowledge, we are the first work that leverages the early exit technique to improve fairness.

% The multi-exit network is designed by putting additional loss constraints at internal exit branches (internal classifier) to increase the accuracy at shallow layer. With the early exit scheme, early exit branches reduce the computational resource during the model inference time while enhancing the model's accuracy. In the inference phase, the instances will stop inferencing and leave the model from different branches following the pre-defined early exit rules or criteria. BranchyNet \cite{teerapittayanon2016branchynet} calculates entropy at each branch after obtaining the result and exits if the entropy of the predicted result is less than the threshold value. Shallow-Deep Networks \cite{kaya2019shallow} calculates the softmax score of each internal classifier's prediction and takes the maximum probability value as the confidence score. Once the score exceeds the threshold during the forward passing, the instance will exit from the branch prematurely.This model further mitigates the ``overthinking'' problem of deep neural networks. \cite{zhou2020bert} makes predictions using adjacent layers and stops inference when the predicted value of the internal classifier remains constant in a given inference unit times. \cite{shrestha2022occamnets} leverage the multi-exit structure to mitigate the dataset bias and improving model predicted power.

% In this paper, we borrow the confidence-based early exit strategy proposed by \cite{kaya2019shallow}to make sure the the early exit instance is confident enough to be correct. To our best knowledge, we are the first work that leverages the early exit technique to improve fairness.


% \subsection{Bias Mitigation Methods}
Bias mitigation methods aim to reduce native bias in datasets and avoid unfair predictions. There are three main approaches to debiasing: pre-processing, in-processing, and post-processing.

Pre-processing strategies adjust training data before training \cite{ngxande2020bias,lu2020gender} or assign different weights to different data samples to suppress the sensitive information during training \cite{kamiran2012data}, but may not be suitable for dermatological data, where the sensitive information needed for diagnosis (such as diseased areas) is present in the images.

In-processing modifies the model architecture, training strategy, and loss function to remove sensitive information\cite{wang2020towards} and achieve fairness, such as adversarial training \cite{alvi2018turning,zhang2018mitigating} or regularization-based \cite{quadrianto2019discovering,jung2021fair} methods. Recently, pruning \cite{wu2022fairprune} techniques have also been used to achieve fairness in dermatological disease diagnosis. However, implementing these methods may result in decreased accuracy for both groups and does not guarantee explicit protection for the unprivileged group when enforcing fairness constraints.

Post-processing techniques aim to enhance fairness by adjusting the model's output distribution to match the training distribution or a specific fairness metric. This calibration is done by taking the model's prediction and the sensitive attribute as inputs \cite{hardt2016equality,zhao2017men,du2020fairness}. Although effective in reducing bias, post-processing methods require access to the sensitive attribute during inference, which may not be feasible for disease diagnosis using image inputs.

In this paper, we propose a general multi-exit (ME) training framework to enhance model fairness without the need to modify data preprocessing or inference strategy, moreover, since the early exit strategy has high confidence in its early exit instances, it does not sacrifice the accuracy of any group and maintains high overall accuracy and fairness simultaneously.

% Bias mitigation methods are designed to reduce the native bias in the dataset to reduce the chance of unfair prediction. There are largely three avenues for current debiased strategy, including pre-processing, in-processing, and post-processing. 

% Pre-processing strategies usually remove the information which may cause ``discrimination'' from training data before training. \cite{kamiran2012data} use different weight to neutralize the effect of the sensitive information in training phase and present the experiments result on real-life data. \cite{ngxande2020bias,lu2020gender} achieve fairness via data pre-process methods including data generation and data augmentation. These strategies are not suitable for dermatological data because the sensitive information which can help diagnosis (i.e., diseased area) in image may be altered or removed.  

% In-processing method usually modify on-the-shelf model architecture, loss function, and model regularization to achieve fairness goal. For example, adversarial training \cite{alvi2018turning,zhang2018mitigating} mitigates the bias through adversarially trains an encoder and classifier to learn a fair representation. Some regularization-based methods, such as \cite{quadrianto2019discovering,jung2021fair} used Hilbert-Schmidt norm and Maximum Mean Discrepancy (MMD) \cite{gretton2012kernel} respectively to learn a fair representation that retain the features' semantics from input domain. Recently, pruning techniques are proved to be an effective method to achieve fairness in dermatological disease diagnosis. \cite{wu2022fairprune} achieve fairness via pruning the parameters that hold large discrepancy of saliencies between different sensitive attributes.

% Post-processing method \cite{hardt2016equality,zhao2017men,du2020fairness} aims to calibrate the model's output to enhance fairness. They need to use sensitive attribute and prediction distribution to modify the previous distribution result. However, these methods need to use sensitive information to achieve fairness, while the disease diagnosis taking images as input.

% Compared with the above methods, we proposed a general bias mitigation framework that could leverage multiple fairness constraints


% Disentangled representation forces the encoder abandon the information of sensitive attributes and thus achieve fairness
%% ?????
% However, those pre-processing and post-processing methods are not suitable for medical image diagnosis task because they need to remove or access sensitive attribute during experiment, it may influence the diagnosis, so our method focus on improving fairness in training phase. Moreover, out method can achieve fairness without knowing sensitive attribute in the training time, which is a "fairness through unawareness" technique.

% However, most pre-processing and post-processing methods are unsuitable for medical image diagnosis tasks because they are required to remove or access sensitive attributes during the experiment, which are not practical. As a result, our method focus on improving fairness in the training phase. Moreover, our method can achieve fairness without knowing sensitive attributes during training, which is a "fairness through unawareness" technique.

==> Table/Compare_SOTA_CelebA.tex <==
\begin{table*}[ht]
\centering
\caption{Classification results of the fairness (EO) and accuracy (Acc.) evaluation on the test set of the CelebA dataset. * denotes our own implementation. }
\setlength{\tabcolsep}{4pt}
\label{Table:Compare_SOTA_CelebA}
\begin{tabular}{c||c|c||c|c||c|c||c|c||c|c||c|c}
\hline
\multirow{2}{*}{Methods}           & \multicolumn{2}{c||}{T=a / S=m} &\multicolumn{2}{c||}{T=a / S=y} &\multicolumn{2}{c||}{T=b / S=m}& \multicolumn{2}{c||}{T=b / S=y}& \multicolumn{2}{c||}{T=e / S=m} & \multicolumn{2}{c}{T=e / S=y}  \\ \cline{2-13}
                  & EO            & Acc.          & EO            & Acc.           & EO           & Acc.          & EO           & Acc.          & EO           & Acc.          & EO           & Acc.          \\ \hline \hline
CNN                   & 27.8          & 79.6          & 16.8          & 79.8           & 17.6         & 84.0          & 14.7         & 84.5          & 15.0         & 83.9          & 12.7         & 83.8          \\ 
\textbf{ME-CNN}       & \textbf{23.7} & \textbf{82.3} & \textbf{16.1} & 76.8           & \textbf{12.9} & \textbf{84.8}         & \textbf{12.9} & \textbf{84.8}         & \textbf{10.8} & 82.5          & \textbf{8.1} & 83.6          \\ \hline
LNL                   & 21.8          & 79.9          & 13.7          & 74.3           & 10.7         & 82.3          & 6.8          & 82.3          & 5.0          & 81.6          & 3.3          & 80.3          \\ 
\textbf{ME-LNL}       & \textbf{14.4} & \textbf{82.2} & \textbf{13.1} & 72.7           & \textbf{7.3} & \textbf{82.8} & \textbf{5.5} & \textbf{83.1} & \textbf{2.7} & \textbf{84.0} & \textbf{1.0} & \textbf{82.6} \\ \hline
HSIC*                 & 19.4          & 81.7          & 16.5          & 80.3           & 11.2         & 80.8          & 10.5         & 82.6          & 12.5         & 84.0          & 7.4          & 84.2          \\ 
\textbf{ME-HSIC}      & \textbf{12.9} & 78.8          & \textbf{15.9} & 78.7           & \textbf{3.6} & \textbf{80.9} & \textbf{3.2} & 82.2          & \textbf{7.8} & 83.5          & \textbf{4.1} & 82.0          \\ \hline
FSCL+                 & 6.5           & 79.1          & 12.4          & 79.1           & 4.7          & 82.9          & 4.8          & 84.1          & 3.0          & 83.4          & 1.6          & 83.5          \\ 
\textbf{ME-FSCL+}     & \textbf{5.8}  & 78.2          & \textbf{7.6}  & 76.4           & \textbf{3.6} & 81.2          & \textbf{2.8} & \textbf{84.4} & \textbf{2.0} & \textbf{83.5} & \textbf{1.4} & 80.8          \\ \hline
MFD                   & 7.4           & 78.0          & 14.9          & 80.0           & 7.3          & 78.0          & 5.4          & 78.0          & 8.7          & 79.0          & 5.2          & 78.0          \\ 
\textbf{ME-MFD}       & \textbf{5.8}  & \textbf{78.3} & \textbf{11.4} & 79.5           & \textbf{2.6} & \textbf{82.1} & \textbf{3.3} & \textbf{82.6} & \textbf{1.4} & \textbf{81.9} & \textbf{1.5} & \textbf{84.2} \\ \hline
% FairPrune             &     21.5          &     81.2          &       22.5         &     82.4           &      17.6        &    83.1           &     15.2         &     83.9          &    17.6  &   83.8            &     9.5         &     84.1          \\ 
% \textbf{ME-FairPrune} &               &               &               &                &             &             &              &               &              &               &              &               \\ \hline
\end{tabular}
\end{table*}

==> Table/Compare_SOTA_UTK.tex <==
% \begin{table}[h]
% \centering
% \caption{Classification results of the fairness (EO) and accuracy (Acc) evaluation on the test set of the CelebA dataset. * denotes our own implementation. $a$, $b$, $e$, $m$, and $y$ respectively denote \emph{Attractive}, \emph{Big Nose}, \emph{Bags Under Eyes}, \emph{Male}, and \emph{Young}. T and S stand for target and sensitive attributes, respectively.}
% \setlength{\tabcolsep}{4pt}
% \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c|c}
% \hline
%     & \multicolumn{10}{|c}{T=Age / S=Ethnicity } & \multicolumn{2}{|c}{T=Gender / S=Ethnicity}        \\ \hline
%     & CNN                 & ME-CNN & LNL* & ME-LNL & HSIC * & ME-HSIC & MFD* & ME-MFD & FairPrune & ME-FairPrune & FSCL*                            & ME-FSCL \\ \hline
% EO  & 17.8                & 15.58  & 18.9 & 16.4   & 16.38  & 14.881  & 15.1 & 13.73  &           &              & 3.7                              & 3.2     \\ \hline
% Acc & 82.4                & 81     & 81.1 & 81.9   & 79.417 & 78.5    & 79.1 & 83.1   &           &              & 70.1                             & 70      \\ \hline
% \end{tabular}
% \end{table}

\begin{table}[h]
% \begin{minipage}{.5\linewidth}
\centering
\caption{Classification results of the fairness (EO) and accuracy (Acc.) evaluation on the test set of the UTK Face dataset. * denotes our own implementation. T and S stand for target and sensitive attributes, respectively. respectively.}
% \setlength{\tabcolsep}{4pt}
\label{Table:Compare_SOTA_UTK}

% \begin{subtable}{.5\linewidth}
% \centering
%     \caption{}
%     \begin{tabular}{c|c|c}
%     \hline
%                                  & \multicolumn{2}{|c}{T=Age / S=Ethnicity}         \\ \hline
%                                  & EO                               & Acc           \\ \hline
%     CNN                          & 17.8                             & 82.4          \\ 
%     \textbf{ME-CNN}              & \textbf{16.0}                    & \textbf{82.5} \\ \hline
%     LNL*                         & 18.9                             & 81.1          \\ 
%     \textbf{ME-LNL}              & \textbf{16.4}                    & \textbf{81.9} \\ \hline
%     HSIC*                        & 16.4                             & 79.4          \\ 
%     \textbf{ME-HSIC}             & \textbf{14.9}                    & 78.5          \\ \hline
%     MFD*                         & 15.1                             & 79.1          \\ 
%     \textbf{ME-MFD}              & \textbf{13.7}                    & \textbf{83.1} \\ \hline
%     % FairPrune                    &                                  &               \\ 
%     % \textbf{ME-FairPrune}        &                                  &               \\ \hline
%     \end{tabular}
% \end{subtable}%
% \begin{subtable}{.5\linewidth}
% \centering
%     \caption{}
%     \begin{tabular}{c|c|c}
%     \hline
%                                  & \multicolumn{2}{|c}{T=Gender / S=Ethnicity}\\ \hline
%                                  & EO                               & Acc  \\ \hline
%     FSCL+*                       & 3.7                              & 70.1 \\ 
%     \textbf{ME-FSCL+}            & \textbf{3.2}                     & 70.0  \\ \hline
    
%     \end{tabular}
% \end{subtable}%
\begin{tabular}{c|c|c|c}
\hline
                              &                             & \multicolumn{2}{c}{S=Ethnicity}         \\ \hline
                              &                             & EO                               & Acc.          \\ \cline{2-4}
\multirow{8}{*}{T=Age}        & CNN*                        & 17.8                             & 82.4          \\ 
                              & \textbf{ME-CNN}             & \textbf{16.0}                    & \textbf{82.5} \\ \cline{2-4}
                              & LNL*                        & 18.9                             & 81.1          \\ 
                              & \textbf{ME-LNL}             & \textbf{16.4}                    & \textbf{81.9} \\ \cline{2-4}
                              & HSIC*                       & 16.4                             & 79.4          \\ 
                              & \textbf{ME-HSIC}            & \textbf{14.9}                    & 78.5          \\ \cline{2-4}
                              & MFD*                        & 15.1                             & 79.1          \\ 
                              & \textbf{ME-MFD}             & \textbf{13.7}                    & \textbf{83.1} \\ \hline
\multirow{2}{*}{T=Gender}     & FSCL+*                      & 3.7                              & 70.1 \\ 
                              & \textbf{ME-FSCL+}           & \textbf{3.2}                     & 70.0  \\ \hline
% FairPrune                    &                                  &               \\ 
% \textbf{ME-FairPrune}        &                                  &               \\ \hline
\end{tabular}
% \end{minipage}

\end{table}



==> Table/comapre.tex <==
\begin{table*}[t]
\centering
\caption{Comparison among the proposed Cfd-CAM, the CAM-based state-of-the-art Grad-CAM\cite{selvaraju2017grad}, Score-CAM\cite{wang2020score}, and LFI-CAM\cite{lee2021lfi} on BraTS dataset with T1, T1-CE, T2, and T2-FLAIR MRI images and TCGA-LGG dataset. Results are reported in the form of mean$\pm$std.}
\label{Table:Compare_Exp_CAM}
\begin{tabular}{l|c|c|c|c|c}
\hline
\multicolumn{6}{c}{BraTS T1} \\ \hline
{\textbf{}}        & \multicolumn{3}{c|}{\textbf{Positive patients}} & \textbf{Negative patients} & \textbf{All patients} \\ \hline
Method           & Dice                  & Precision             & Recall                & Dice                       & Dice             \\ \hline
Grad-CAM\cite{selvaraju2017grad}        & 0.107$\pm$0.090          & 0.060$\pm$0.057          & 0.692$\pm$0.377          & 0.000$\pm$0.000               & 0.046$\pm$0.079          \\ \hline
ScoreCAM\cite{wang2020score}        & 0.296$\pm$0.128          & 0.183$\pm$0.090          & \textbf{0.887$\pm$0.244}          & 0.136$\pm$0.342               & 0.205$\pm$0.283          \\ \hline
LFI-CAM\cite{lee2021lfi}         & 0.437$\pm$0.243          & \textbf{0.494$\pm$0.342}          & 0.592$\pm$0.272          & 0.000$\pm$0.000               & 0.188$\pm$0.269          \\ \hline
Cfd-CAM (ours)   & \textbf{0.438$\pm$0.172} & 0.312$\pm$0.148 & 0.849$\pm$0.250 & \textbf{0.929$\pm$0.257}      & \textbf{0.718$\pm$0.331} \\ \hline \hline
\multicolumn{6}{c}{BraTS T1-CE} \\ \hline
{\textbf{}}        & \multicolumn{3}{c|}{\textbf{Positive patients}} & \textbf{Negative patients} & \textbf{All patients} \\ \hline
Method           & Dice                  & Precision             & Recall                & Dice                       & Dice             \\ \hline
Grad-CAM\cite{selvaraju2017grad}        & 0.127$\pm$0.088          & 0.072$\pm$0.055          & 0.795$\pm$0.282          & 0.000$\pm$0.000               & 0.057$\pm$0.086          \\ \hline
ScoreCAM\cite{wang2020score}        & 0.397$\pm$0.188          & 0.289$\pm$0.200          & \textbf{0.926$\pm$0.160}          & 0.135$\pm$0.341               & 0.253$\pm$0.311          \\ \hline
LFI-CAM\cite{lee2021lfi}         & 0.029$\pm$0.066          & 0.016$\pm$0.038          & 0.133$\pm$0.297          & 0.000$\pm$0.000               & 0.013$\pm$0.047          \\ \hline
Cfd-CAM (ours)   & \textbf{0.600$\pm$0.192} & \textbf{0.543$\pm$0.235} & 0.785$\pm$0.237 & \textbf{0.944$\pm$0.230}      & \textbf{0.789$\pm$0.274} \\ \hline \hline
\multicolumn{6}{c}{BraTS T2} \\ \hline
{\textbf{}}        & \multicolumn{3}{c|}{\textbf{Positive patients}} & \textbf{Negative patients} & \textbf{All patients} \\ \hline
Method           & Dice                  & Precision             & Recall                & Dice                       & Dice             \\ \hline
Grad-CAM\cite{selvaraju2017grad}         & 0.048$\pm$0.058          & 0.027$\pm$0.037          & 0.443$\pm$0.409          & 0.000$\pm$0.000               & 0.023$\pm$0.047          \\ \hline
ScoreCAM\cite{wang2020score}         & 0.529$\pm$0.183          & 0.400$\pm$0.195          & 0.932$\pm$0.132          & 0.135$\pm$0.341               & 0.323$\pm$0.340          \\ \hline
LFI-CAM\cite{lee2021lfi}          & \textbf{0.685$\pm$0.201}          & \textbf{0.708$\pm$0.276}          & 0.768$\pm$0.179          & 0.000$\pm$0.000               & 0.327$\pm$0.369          \\ \hline
Cfd-CAM (ours)   & 0.646$\pm$0.157 & 0.570$\pm$0.201 & \textbf{0.826$\pm$0.164} & \textbf{0.929$\pm$0.257}      & \textbf{0.794$\pm$0.257} \\ \hline \hline
\multicolumn{6}{c}{BraTS T2-FLAIR} \\ \hline
{\textbf{}}        & \multicolumn{3}{c|}{\textbf{Positive patients}} & \textbf{Negative patients} & \textbf{All patients} \\ \hline
Method           & Dice                  & Precision             & Recall                & Dice                       & Dice             \\ \hline
Grad-CAM\cite{selvaraju2017grad}        & 0.150$\pm$0.076          & 0.083$\pm$0.050          & 0.991$\pm$0.057          & 0.000$\pm$0.000               & 0.072$\pm$0.092          \\ \hline
ScoreCAM\cite{wang2020score}        & 0.431$\pm$0.209          & 0.314$\pm$0.202          & \textbf{0.890$\pm$0.232}          & 0.135$\pm$0.341               & 0.279$\pm$0.321          \\ \hline
LFI-CAM\cite{lee2021lfi}         & 0.674$\pm$0.175          & 0.648$\pm$0.236          & 0.806$\pm$0.179          & 0.000$\pm$0.000               & 0.328$\pm$0.358          \\ \hline
Cfd-CAM (ours)   & \textbf{0.691$\pm$0.182} & \textbf{0.656$\pm$0.238} & 0.814$\pm$0.197 & \textbf{0.981$\pm$0.137}      & \textbf{0.840$\pm$0.216} \\ \hline \hline
\multicolumn{6}{c}{TCGA-LGG} \\ \hline
{\textbf{}}        & \multicolumn{3}{c|}{\textbf{Positive patients}} & \textbf{Negative patients} & \textbf{All patients} \\ \hline
Method           & Dice                  & Precision             & Recall                & Dice                       & Dice             \\ \hline
Grad-CAM\cite{selvaraju2017grad}        & 0.257$\pm$0.197          & 0.204$\pm$0.182          & 0.481$\pm$0.341          & 0.983$\pm$0.130               & 0.746$\pm$0.374          \\ \hline
ScoreCAM\cite{wang2020score}        & 0.492$\pm$0.230          & 0.512$\pm$0.277          & \textbf{0.596$\pm$0.275}          & 0.983$\pm$0.130               & 0.755$\pm$0.249         \\ \hline
LFI-CAM\cite{lee2021lfi}         & 0.460$\pm$0.245          & 0.689$\pm$0.333          & 0.392$\pm$0.250          & 0.000$\pm$0.000               & 0.150$\pm$0.257          \\ \hline
Cfd-CAM (ours) & \textbf{0.546$\pm$0.245}   & \textbf{0.630$\pm$0.285} & \textbf{0.559$\pm$0.291} & \textbf{0.986$\pm$0.118}      & \textbf{0.842$\pm$0.267} \\ \hline
\end{tabular}
\end{table*}

==> Table/merge_SOTA_ME_compare.tex <==
\begin{table}[ht]
\centering
\label{Table:compare_merge}
\scriptsize
\begin{tabular}{N N N N N N N N N N N N N N N N}\toprule
\multicolumn{1}{N }{\text{}} & \multicolumn{1}{c }{\text{}} &\multicolumn{3}{c }{\text{Accuracy}} & \multicolumn{3}{c }{\text{Fairness}}  \multicolumn{1}{N }{\text{}} & \multicolumn{1}{c }{\text{}} &\multicolumn{3}{c }{\text{Accuracy}} & \multicolumn{3}{c }{\text{Fairness}}\\ 
\cmidrule(lr){3-5}
\cmidrule(ll){6-8}
\cmidrule(ll){9-9}
\cmidrule(ll){10-10}
\cmidrule(ll){11-13}
\cmidrule(ll){14-16}
\multicolumn{1}{ c }{\text{Method}} & \text{Gender} &\text{Precision} & \text{Recall} & \text{F1-score} & \text{Eopp0} & \text{Eopp1} & \text{Eodd} {\text{Method}} & \text{Skin Tone} &\text{Precision} & \text{Recall} & \text{F1-score} & \text{Eopp0} & \text{Eopp1} & \text{Eodd}\\ 
\cmidrule(lr){1-1}
\cmidrule(lr){2-2}
\cmidrule(lr){3-5}
\cmidrule(ll){6-8}
\cmidrule(ll){9-9}
\cmidrule(ll){10-10}
\cmidrule(ll){11-13}
\cmidrule(ll){14-16}
\multirow{8}{*}{\multicolumn{1}{ c }{ResNet18}} & \text{Female} & 0.793 & 0.721 & 0.746 & \multirow{4}{*}{0.006} & \multirow{4}{*}{0.044} & \multirow{4}{*}{0.022} {\multicolumn{1}{ c }{VGG11}} & \text{Dark} & 0.563 & 0.581 & 0.546 & \multirow{4}{*}{0.0013} & \multirow{4}{*}{0.361} & \multirow{4}{*}{0.182} \\ 
 & \text{Male} & 0.731 & 0.725 & 0.723 &  &  & \text{Light} & 0.482 & 0.495 & 0.473 &  &  & \\ 
 & \text{Avg.} & 0.762 & 0.723 & 0.735 &  &  & \text{Avg.} & 0.523 & 0.538 & 0.510 &  &  &  \\ 
 & \text{Diff.} & 0.063 & 0.004 & 0.023 &  &  & \text{Diff.} & 0.081 & 0.086 & 0.073 &  &  &  \\ 
\hline

\multirow{4}{*}{\multicolumn{1}{ c }{AdvConf}} & \text{Female} & 0.755 & 0.738 & 0.741 & \multirow{4}{*}{0.008} & \multirow{4}{*}{0.070} & \multirow{4}{*}{0.037} \\ 
 & \text{Male} & 0.710 & 0.757 & 0.731 &  &  & \\ 
 & \text{Avg.} & 0.733 & 0.747 & 0.736 &  &  & \\ 
 & \text{Diff.} & 0.045 & 0.020 & 0.010 &  &  & \\ 
\hline
\multirow{4}{*}{\multicolumn{1}{ c }{AdvRev}} & \text{Female} & 0.778 & 0.683 & 0.716 & \multirow{4}{*}{0.007} & \multirow{4}{*}{0.059} & \multirow{4}{*}{0.033} \\ 
 & \text{Male} & 0.773 & 0.706 & 0.729 &  &  & \\ 
 & \text{Avg.} & 0.775 & 0.694 & 0.723 &  &  & \\ 
 & \text{Diff.} & 0.006 & 0.023 & 0.014 &  &  & \\ 
\hline
\multirow{4}{*}{\multicolumn{1}{ c }{DomainIndep}} & \text{Female} & 0.729 & 0.747 & 0.734 & \multirow{4}{*}{0.010} & \multirow{4}{*}{0.086} & \multirow{4}{*}{0.042} \\ 
 & \text{Male} & 0.725 & 0.694 & 0.702 &  &  & \\ 
 & \text{Avg.} & 0.727 & 0.721 & 0.718 &  &  & \\ 
 & \text{Diff.} & 0.004 & 0.053 & 0.031 &  &  & \\ 
\hline

\multirow{4}{*}{\multicolumn{1}{ c }{HSIC}} & \text{Female} & 0.744 & 0.660 & 0.696 & \multirow{4}{*}{0.008} & \multirow{4}{*}{0.042} & \multirow{4}{*}{0.019} \\ 
 & \text{Male} & 0.718 & 0.697 & 0.705 &  &  & \\ 
 & \text{Avg.} & 0.731 & 0.679 & 0.700 &  &  & \\ 
 & \text{Diff.} & 0.026 & 0.037 & 0.009 &  &  & \\ 
\hline

% \multicolumn{1}{ c }{HSIC} & 0.74 & 15 & 630 & 0.70 & 15 & 618 & -\\ 
\multirow{4}{*}{\multicolumn{1}{ c }{MFD}} & \text{Female} & 0.770 & 0.697 & 0.727 & \multirow{4}{*}{0.005} & \multirow{4}{*}{0.051} & \multirow{4}{*}{0.024} \\ 
 & \text{Male} & 0.772 & 0.726 & 0.744 &  &  & \\ 
 & \text{Avg.} & 0.771 & 0.712 & 0.736 &  &  & \\ 
 & \text{Diff.} & 0.002 & 0.029 & 0.017 &  &  & \\ 
\hline

% \multicolumn{1}{ c }{MFD} & 0.06 & 7 & 21 & 0.06 & 5 & 27 & -\\ 
% \multirow{4}{*}{\multicolumn{1}{ c }{DomainIndep}} & \text{Female} & 0.729 & 0.747 & 0.734 & \multirow{4}{*}{0.010} & \multirow{4}{*}{0.086} & \multirow{4}{*}{0.042} \\ 
%  & \text{Male} & 0.725 & 0.694 & 0.702 &  &  & \\ 
%  & \text{Avg.} & 0.727 & 0.721 & 0.718 &  &  & \\ 
%  & \text{Diff.} & 0.004 & 0.053 & 0.031 &  &  & \\ 
% \hline
% \multicolumn{1}{ c }{DomainIndep} & 0.06 & 7 & 21 & 0.06 & 5 & 27 & -\\ 
\multirow{4}{*}{\multicolumn{1}{ c }{FairPrune}} & \text{Female} & 0.776 & 0.711 & 0.734 & \multirow{4}{*}{0.007} & \multirow{4}{*}{0.026} & \multirow{4}{*}{0.014} \\ 
 & \text{Male} & 0.721 & 0.725 & 0.720 &  &  & \\ 
 & \text{Avg.} & 0.748 & 0.718 & 0.727 &  &  & \\ 
 & \text{Diff.} & 0.055 & 0.014 & 0.014 &  &  & \\ 
\hline
% \multicolumn{1}{ c }{FairPrune} & 0.06 & 7 & 21 & 0.06 & 5 & 27 & -\\ 
\multirow{4}{*}{\multicolumn{1}{ c }{ME-FairPrune}} & \text{Female} & 0.770 & \textbf{0.723} & 0.742 & \multirow{4}{*}{0.006} & \multirow{4}{*}{\textbf{0.020}} & \multirow{4}{*}{\textbf{0.010}} \\ 
 & \text{Male} & 0.739 & 0.728 & 0.730 &  &  & \\ 
 & \text{Avg.} & 0.755 & 0.725 & 0.736 &  &  & \\ 
 & \text{Diff.} & 0.032 & 0.005 & 0.012 &  &  & \\ 
\bottomrule
\end{tabular}
\end{table}


% \begin{tabular}{SSSSSSSS} 
% \toprule
% \multicolumn{7}{c}{Accuracy} {Fairness}\\
% \cmidrule(r){3-5} \cmidrule(lr){6-8}
%     {Method} & {Skin Tone} & {Precision} & {Recall} & {F1-score} & {Eopp0} & {Eopp1} & {Eodd} \\ \midrule
%     1  & 16.128 & +8.872 & 16.128 & 1.402 & 1.373 & -146.6 & -137.6 \\
%     2  & 3.442  & -2.509 & 3.442  & 0.299 & 0.343 & 133.2  & 152.4  \\
%     3  & 1.826  & -0.363 & 1.826  & 0.159 & 0.119 & 168.5  & -161.1 \\
%     4  & 0.993  & -0.429 & 0.993  & 0.086 & 0.08  & 25.6   & 90     \\ \midrule
%     5  & 1.29   & +0.099 & 1.29   & 0.112 & 0.097 & -175.6 & -114.7 \\
%     6  & 0.483  & -0.183 & 0.483  & 0.042 & 0.063 & 22.3   & 122.5  \\
%     7  & 0.766  & -0.475 & 0.766  & 0.067 & 0.039 & 141.6  & -122   \\
%     8  & 0.624  & +0.365 & 0.624  & 0.054 & 0.04  & -35.7  & 90     \\ \midrule
%     9  & 0.641  & -0.466 & 0.641  & 0.056 & 0.045 & 133.3  & -106.3 \\
%     10 & 0.45   & +0.421 & 0.45   & 0.039 & 0.034 & -69.4  & 110.9  \\
%     11 & 0.598  & -0.597 & 0.598  & 0.052 & 0.025 & 92.3   & -109.3 \\ \bottomrule
% \end{tabular}


==> Table/supp_compare_isic_vgg.tex <==
\begin{table}[ht]
\centering
\caption{Results of accuracy and fairness of different methods on ISIC 2019 dataset, using gender as the sensitive attribute. The female is the privileged group with higher accuracy by vanilla training. All results are our implementation. }
\setlength{\tabcolsep}{6pt}
\label{Table:compare_isic}
\scriptsize
\begin{tabular}{c c c c c c c c}\toprule 
% \hline
% {\multirow{2}{*}{Method}} & \multicolumn{1}{c@{}}{\multirow{2}{*}{Gender}} &\multicolumn{3}{c@{}}{\text{Accuracy}} & \multicolumn{3}{c}{\text{Fairness}}  \\ 
% \cmidrule(lr){3-5}
% \cmidrule(ll){6-8}
% {} & {} &\text{Precision} & \text{Recall} & \text{F1-score} & \text{Eopp0 $\downarrow$} & \text{Eopp1 $\downarrow$} & \text{Eodd $\downarrow$} \\ 
% \cmidrule(lr){1-1}
% \cmidrule(lr){2-2}
% \cmidrule(lr){3-5}
% \cmidrule(ll){6-8}
\multicolumn{1}{c }{\text{}} & \multicolumn{1}{c }{\text{}} &\multicolumn{3}{c }{\text{Accuracy}} & \multicolumn{3}{c }{\text{Fairness}}  \\ 
\cmidrule(lr){3-5}
\cmidrule(ll){6-8}
\multicolumn{1}{ c }{\text{Method}} & \text{Gender} &\text{Precision} & \text{Recall} & \text{F1-score} & \text{Eopp0 $\downarrow$} & \text{Eopp1 $\downarrow$} & \text{Eodd $\downarrow$} \\ 
\hline
\hline
 {\multirow{4}{*}{VGG11}} & \text{Female} & 0.793 & 0.721 & 0.746 & \multirow{4}{*}{0.006} & \multirow{4}{*}{0.044} & \multirow{4}{*}{0.022} \\ 
 & \text{Male} & 0.731 & 0.725 & 0.723 &  &  & \\ 
 & \text{Avg. $\uparrow$} & 0.762 & 0.723 & 0.735 &  &  & \\ 
 & \text{Diff. $\downarrow$} & 0.063 & 0.004 & 0.023 &  &  & \\ 
% \hline
% \cmidrule(lr){1-1}
% \cmidrule(lr){2-2}
% \cmidrule(lr){3-5}
% \cmidrule(ll){6-8}

% \multirow{4}{*}{\multicolumn{1}{ c }{ME-ResNet18}} & \text{Female} & 0.748 & 0.724 & 0.733 & \multirow{4}{*}{0.006} & \multirow{4}{*}{0.031} & \multirow{4}{*}{0.016} \\ 
%  & \text{Male} & 0.723 & 0.736 & 0.726 &  &  & \\ 
%  & \text{Avg.} & 0.735 & 0.730 & 0.730 &  &  & \\ 
%  & \text{Diff.} & 0.025 & 0.012 & 0.007 &  &  & \\ 
% \hline
\hline


\multirow{4}{*}{AdvConf} & \text{Female} & 0.755 & 0.738 & 0.741 & \multirow{4}{*}{0.008} & \multirow{4}{*}{0.070} & \multirow{4}{*}{0.037} \\ 
 & \text{Male} & 0.710 & 0.757 & 0.731 &  &  & \\ 
 & \text{Avg. $\uparrow$} & 0.733 & 0.747 & 0.736 &  &  & \\ 
 & \text{Diff. $\downarrow$} & 0.045 & 0.020 & 0.010 &  &  & \\ 
\hline
% \cmidrule(lr){1-1}
% \cmidrule(lr){2-2}
% \cmidrule(lr){3-5}
% \cmidrule(ll){6-8}
\multirow{4}{*}{AdvRev} & \text{Female} & 0.778 & 0.683 & 0.716 & \multirow{4}{*}{0.007} & \multirow{4}{*}{0.059} & \multirow{4}{*}{0.033} \\ 
 & \text{Male} & 0.773 & 0.706 & 0.729 &  &  & \\ 
 & \text{Avg. $\uparrow$} & 0.775 & 0.694 & 0.723 &  &  & \\ 
 & \text{Diff. $\downarrow$} & 0.006 & 0.023 & 0.014 &  &  & \\ 
%  \cmidrule(lr){1-1}
% \cmidrule(lr){2-2}
% \cmidrule(lr){3-5}
% \cmidrule(ll){6-8}
\hline
\multirow{4}{*}{DomainIndep} & \text{Female} & 0.729 & 0.747 & 0.734 & \multirow{4}{*}{0.010} & \multirow{4}{*}{0.086} & \multirow{4}{*}{0.042} \\ 
 & \text{Male} & 0.725 & 0.694 & 0.702 &  &  & \\ 
 & \text{Avg. $\uparrow$} & 0.727 & 0.721 & 0.718 &  &  & \\ 
 & \text{Diff. $\downarrow$} & 0.004 & 0.053 & 0.031 &  &  & \\ 
% \hline
\hline
\multirow{4}{*}{HSIC} & \text{Female} & 0.744 & 0.660 & 0.696 & \multirow{4}{*}{0.008} & \multirow{4}{*}{0.042} & \multirow{4}{*}{0.020} \\ 
 & \text{Male} & 0.718 & 0.697 & 0.705 &  &  & \\ 
 & \text{Avg. $\uparrow$} & 0.731 & 0.679 & 0.700 &  &  & \\ 
 & \text{Diff. $\downarrow$} & 0.026 & 0.037 & 0.009 &  &  & \\ 
% \cmidrule(lr){1-1}
% \cmidrule(lr){2-2}
% \cmidrule(lr){3-5}
% \cmidrule(ll){6-8}
% % \hline

% \multirow{4}{*}{\multicolumn{1}{ c }{ME-HSIC}} & \text{Female} & 0.733 & 0.707 & 0.716 & \multirow{4}{*}{0.007} & \multirow{4}{*}{0.034} & \multirow{4}{*}{0.018} \\ 
%  & \text{Male} & 0.713 & 0.707 & 0.707 &  &  & \\ 
%  & \text{Avg.} & 0.723 & 0.707 & 0.712 &  &  & \\ 
%  & \text{Diff.} & 0.020 & 0.000 & 0.009 &  &  & \\ 
% \hline
\hline
% \multicolumn{1}{ c }{HSIC} & 0.74 & 15 & 630 & 0.70 & 15 & 618 & -\\ 
\multicolumn{1}{ c }{\multirow{4}{*}{MFD}} & \text{Female} & 0.770 & 0.697 & 0.726 & \multirow{4}{*}{\textbf{0.005}} & \multirow{4}{*}{0.051} & \multirow{4}{*}{0.024} \\ 
 & \text{Male} & 0.772 & 0.726 & 0.744 &  &  & \\ 
 & \text{Avg. $\uparrow$} & 0.771 & 0.712 & 0.735 &  &  & \\ 
 & \text{Diff. $\downarrow$} & 0.002 & 0.029 & 0.018 &  &  & \\ 
% \hline
% \cmidrule(lr){1-1}
% \cmidrule(lr){2-2}
% \cmidrule(lr){3-5}
% \cmidrule(ll){6-8}

% \multirow{4}{*}{\multicolumn{1}{ c }{ME-MFD}} & \text{Female} & 0.733 & 0.698 & 0.711 & \multirow{4}{*}{0.006} & \multirow{4}{*}{0.024} & \multirow{4}{*}{0.012} \\ 
%  & \text{Male} & 0.772 & 0.713 & 0.739 &  &  & \\ 
%  & \text{Avg.} & 0.752 & 0.706 & 0.725 &  &  & \\ 
%  & \text{Diff.} & 0.039 & 0.015 & 0.028 &  &  & \\ 
\hline
\hline
% \multicolumn{1}{ c }{MFD} & 0.06 & 7 & 21 & 0.06 & 5 & 27 & -\\ 
% \multirow{4}{*}{\multicolumn{1}{ c }{DomainIndep}} & \text{Female} & 0.729 & 0.747 & 0.734 & \multirow{4}{*}{0.010} & \multirow{4}{*}{0.086} & \multirow{4}{*}{0.042} \\ 
%  & \text{Male} & 0.725 & 0.694 & 0.702 &  &  & \\ 
%  & \text{Avg.} & 0.727 & 0.721 & 0.718 &  &  & \\ 
%  & \text{Diff.} & 0.004 & 0.053 & 0.031 &  &  & \\ 
% \hline
% \multicolumn{1}{ c }{DomainIndep} & 0.06 & 7 & 21 & 0.06 & 5 & 27 & -\\ 
{\multirow{4}{*}{FairPrune}} & \text{Female} & 0.776 & 0.711 & 0.734 & \multirow{4}{*}{0.007} & \multirow{4}{*}{0.026} & \multirow{4}{*}{0.014} \\ 
 & \text{Male} & 0.721 & 0.725 & 0.720 &  &  & \\ 
 & \text{Avg. $\uparrow$} & 0.748 & 0.718 & 0.727 &  &  & \\ 
 & \text{Diff. $\downarrow$} & 0.055 & 0.014 & 0.014 &  &  & \\ 
\hline

\multicolumn{1}{ c }{\multirow{4}{*}{ME-FairPrune}} & \text{Female} & 0.770 & 0.723 & 0.742 & \multirow{4}{*}{0.006} & \multirow{4}{*}{\textbf{0.020}} & \multirow{4}{*}{\textbf{0.010}} \\ 
 & \text{Male} & 0.739 & 0.728 & 0.730 &  &  & \\ 
 & \text{Avg. $\uparrow$} & 0.755 & 0.725 & 0.736 &  &  & \\ 
 & \text{Diff. $\downarrow$} & 0.032 & 0.005 & 0.012 &  &  & \\ 
 % \hline
\bottomrule
\end{tabular}
\end{table}


